Personalized Safety in LLMs: A Benchmark and A Planning-Based Agent Approach

Large language models (LLMs) typically generate identical or similar responses for all users given the same prompt, posing serious safety risks in high-stakes applications where user vulnerabilities differ widely. Existing safety evaluations primarily rely on context-independent metrics - such as factuality, bias, or toxicity - overlooking the fact that the same response may carry divergent risks depending on the user's background or condition. We introduce personalized safety to fill this gap and present PENGUIN - a benchmark comprising 14,000 scenarios across seven sensitive domains with both context-rich and context-free variants. Evaluating six leading LLMs, we demonstrate that personalized user information significantly improves safety scores by 43.2%, confirming the effectiveness of personalization in safety alignment. However, not all context attributes contribute equally to safety enhancement. To address this, we develop RAISE - a training-free, two-stage agent framework that strategically acquires user-specific background. RAISE improves safety scores by up to 31.6% over six vanilla LLMs, while maintaining a low interaction cost of just 2.7 user queries on average. Our findings highlight the importance of selective information gathering in safety-critical domains and offer a practical solution for personalizing LLM responses without model retraining. This work establishes a foundation for safety research that adapts to individual user contexts rather than assuming a universal harm standard.

==> CheckList.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The abstract and introduction clearly and accurately summarize the paper’s key contributions: (1) defining the problem of personalized safety for LLMs, (2) introducing the PENGUIN benchmark with 14,000 personalized high-risk scenarios, and (3) proposing the RAISE agent framework to optimize context acquisition under limited interaction budgets. These components are consistently expanded upon in Sections 3–5.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The limitations are explicitly discussed in Section 6 (Conclusions, Limitations, and Societal Impact). The authors mention two key limitations: 1. The method assumes uniform cost across all user attributes, which may not reflect the real-world difficulty of acquiring different kinds of personal information. 2. The system currently relies on manually defined attributes; future work could explore automatic discovery and abstraction to enhance scalability.

These limitations are clearly acknowledged, contextualized, and provide useful directions for future research.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper presents a theoretical result related to the convergence of the LLM-guided Monte Carlo Tree Search (MCTS) used in the RAISE framework. As stated in Section 5.2 and referenced in Appendix C.7, the authors provide the formal convergence analysis of their LLM-guided MCTS algorithm, including the necessary assumptions (e.g., bounded rewards) and a complete sketch of the proof. This validates that the planning module retains asymptotic optimality and ensures theoretical soundness.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide the same evaluation framework and code used in our experiments to enable other researchers to reproduce and build upon our work. Our framework is easy to use—researchers simply specify the models they wish to test and receive results directly.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes. As stated in the supplemental material (Appendix A.4 and B.3), the authors plan to release the full PENGUIN benchmark (14,000 annotated scenarios) along with the RAISE framework implementation upon publication. The supplemental material includes data preprocessing procedures, attribute extraction protocols, model evaluation setup, and ablation details, ensuring that the main results can be faithfully reproduced. Full instructions for dataset use, model configuration, and evaluation scripts are provided.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We detail all models and settings used in our experiments in Section~\ref{sec-exp-details}, including the specific model variants and token sampling strategies, to ensure the reproducibility of our results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper analyzes the convergence behavior of LLM-guided MCTS in Appendix C.3—including performance stability and convergence speed.
    \item[] Guidelines: 
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We specify that we used 8xA100 and 2xH100 GPUs over the course of 2 weeks in our Experimental Details section of our paper in \ref{sec-exp-details}.}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes. The paper adheres to NeurIPS ethical guidelines in all aspects. It addresses potential risks of LLMs in high-stakes scenarios, such as mental health, finances, and social vulnerability, and proposes mechanisms (e.g., RAISE framework and abstention module) to mitigate harm through personalized and cautious generation.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes. The paper discusses positive societal impacts such as enabling safer and more responsible deployment of large language models in high-risk domains like mental health, career counseling, and financial advising (see Section 6: Conclusions, Limitations, and Societal Impact). It emphasizes how personalized safety mechanisms can prevent harm and support vulnerable users through adaptive, empathetic responses.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer:  \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes. The paper includes multiple safeguards for the responsible release of its PENGUIN benchmark, which involves potentially sensitive user scenarios: 1. Real-world data is sourced from Reddit via the PushShift API, and all posts undergo structured extraction, safety filtering, and human verification to ensure removal of unsafe, offensive, or personally identifiable content (see Appendix A.4). 2. Synthetic data is generated under relational constraints to ensure coherence, and manually reviewed to eliminate any unsafe prompts or hallucinations, following best practices in toxic content filtering).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes. The paper properly credits all external assets used in the research. For example: Language models such as GPT-4o, LLaMA-3, Mistral-7B, Qwen, and Deepseek-7B are clearly named, and relevant technical reports or system cards are cited (e.g., [41], [45], [24]). Reddit data is collected via the PushShift API [4], and the authors cite the appropriate source and follow data ethics protocols (Appendix A.4). Prior benchmarks and tools used for alignment evaluation, safety testing, or data filtering are also cited (e.g., RealToxicityPrompts [18], EmpatheticDialogues [47]).

    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes. The paper introduces two major new assets: PENGUIN benchmark – a dataset of 14,000 high-risk user scenarios across seven domains. RAISE agent framework – a training-free, planning-based system for personalized context acquisition.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes. We provide the full text of annotation instructions used during human evaluation in Appendix B.1. Annotators were graduate-level research assistants trained by the authors. No monetary compensation was provided, as all participants volunteered as part of a university research project.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This study does not involve intervention or collection of personal information from human subjects. All annotation tasks were conducted by trained research assistants. According to our institution's guidelines, this study does not qualify as human subjects research and does not require IRB approval.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes. The usage of LLMs is a core and novel component of this work. Specifically, the paper introduces a two-stage agent framework (RAISE) where LLMs are used both for simulating user-aware response generation and for guiding the Monte Carlo Tree Search (MCTS) during offline path planning. The paper also employs LLMs (e.g., GPT-4o) as oracles for safety scoring, and uses them to generate synthetic high-risk scenarios. These usages go beyond typical applications and are thoroughly documented in Sections 3, 4, and 5, as well as Appendix C.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> Data.tex <==
\section{Personalized Safety Dataset Construction}\label{sec:data}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/data.jpg}
    \caption{Data construction and collection process}
    \label{fig:dataset_construction}
\end{figure}

%In this section, we describe the data construction process of the Personalized Safety Benchmark, which is designed to evaluate how well large language models (LLMs) respond to user scenarios involving high emotional stakes and personalized safety risks.To ensure both realism and diversity, we construct samples from Reddit communities associated with high-risk domains such as finance, relationships, and mental health. These user posts are filtered and structured using GPT-4o to ensure sufficient contextual detail and attribute coverage. In addition, we generate synthetic scenarios using domain-specific prompts, allowing us to control for rare demographic combinations and balance attribute distributions across domains.
To systematically evaluate the personalized safety performance of large language models in high-risk and emotionally sensitive contexts, we design a multi-source data construction process.
Our benchmark dataset integrates two types of data sources: real-world user posts collected from Reddit and synthetic scenarios generated through domain-specific prompting strategies.
Real-world data enhances realism by providing natural language expression and authentic vulnerability contexts, while synthetic data enables systematic expansion to rare scenarios, controlled background variables, and reduces the risk of training data contamination.
The complete data collection and processing pipeline is illustrated in Figure~\ref{fig:dataset_construction}, with each component detailed in the following subsections. 

\subsection{Reddit-Based Data Generation}
To ensure the systematicity and reproducibility of our methodology, we establish a unified data processing pipeline consisting of three stages: data acquisition, sample selection, and data construction. We first use the Reddit PushShift API\cite{baumgartner2020pushshiftredditdataset} to collect posts from 2019 to 2025 across the most active subreddits in each domain, gathering approximately 250,000 anonymized posts per subreddit. For each post, we use a structured prompt with GPT-4o (details in Appendix) to extract ten predefined user background attributes.

During filtering, we retain only posts that cover at least 7 out of the 10 attributes, ensuring sufficient richness of user background information. The threshold of 7 attributes was determined based on preliminary analysis: requiring at least 7 attributes strikes a balance between background completeness and sample size. In particular, while setting a higher threshold (e.g., 9 or 10 attributes) would drastically reduce the available data to impractically small amounts, setting a lower threshold (e.g., 5 or fewer) would result in insufficient context for reliable downstream evaluation. This balance is critical, as even with the 7-attribute threshold, only approximately 0.4% of the collected posts meet the criteria in our dataset, emphasizing the need for large-scale collection and automatic structured extraction.

Manual annotation under such sparsity would be prohibitively costly and unscalable. Therefore, we leverage large language model (LLM)-assisted structured information extraction to efficiently infer and filter high-quality samples. Our full extraction and filtering pipeline adheres to recent best practices in LLM-based structured information extraction~\cite{yuan2025sevalautomatedcomprehensivesafety, tan2025judgebenchbenchmarkevaluatingllmbased, xiao2024rnagptmultimodalgenerativerna}, and incorporates consistency checks to ensure scalability, reliability, and reproducibility of the final dataset.


\subsection{Synthetic Data Generation}
While real-world Reddit scenarios provide valuable authenticity, they also pose a risk of data contamination—especially for LLMs trained on extensive web corpora. Prior work has shown that many benchmark datasets derived from online sources may appear, either verbatim or paraphrased, in pretraining data~\cite{zhu2024dyvaldynamicevaluationlarge}. This can lead to inflated evaluations and unreliable conclusions. To mitigate this concern, we construct a parallel set of synthetic samples using a constraint-driven generation pipeline, ensuring that evaluation scenarios remain out-of-distribution with respect to model pretraining data.

\textbf{Structured Background Construction.}
Each user background is represented as a structured profile composed of ten attributes that are sampled under two types of constraints: \textbf{Global constraints}, which restrict each field to a valid range or category set (e.g., age between 18–65). \textbf{Relational constraints}, which enforce semantic coherence between fields (e.g., profession depends on education level and age group). GPT-4o is used to sample attribute values under these constraints, ensuring semantic coherence and diversity across user profile.

\textbf{Query Generation.}
Given a synthesized user background, we employ GPT-4o with domain-specific prompts to generate multiple high-risk queries reflecting realistic concerns grounded in the background context.
Each profile yields 10 queries to capture different facets of potential emotional vulnerability or decision-making pressure. The overall process is shown in Figure \ref{fig:dataset_construction}.

%To construct personalized high-risk scenarios grounded in real-world user experience, we collect posts from Reddit, a large-scale social platform where users frequently seek guidance on emotionally charged and high-stakes life decisions. We target seven domains consistently associated with psychological vulnerability and complex personal circumstances: \textit{relationships}, \textit{career}, \textit{financial}, \textit{social}, \textit{health}, \textit{life decisions}, and \textit{education}. For each domain, we select 2–4 representative subreddits based on relevance, post volume, and community engagement, as shown in the Table~\ref{tab:domain-subreddits}.

%We collect posts published between 2019 and 2025 from the selected subreddits. To ensure that each scenario contains sufficient background detail for personalized safety evaluation, we retain only posts that include a clear user query and cover at least 7 out of 10 predefined background attributes, either explicitly stated or reasonably inferable. Given the sparsity of Reddit posts containing sufficiently rich background information (only 2–3\% of raw data), we adopt GPT-4o to assist with attribute inference and filtering—a decision informed by recent studies demonstrating that large language models can reliably perform structured information extraction and content-level judgments~\cite{yuan2025sevalautomatedcomprehensivesafety, tan2025judgebenchbenchmarkevaluatingllmbased, xiao2024rnagptmultimodalgenerativerna}.

%\textbf{Structured Background Generation.}
%We define a generation function \( G \) that produces structured user profiles \( U_i \) based on two sets of constraints: global attribute ranges (\( C_{\text{Global}} \)) and relational dependencies (\( C_{\text{Relational}} \)). Global constraints specify valid value ranges for each attribute (e.g., $\text{age} \in [18\text{--}65]$, education \( \in \) \{high school, college, master's\}), while relational constraints encode dependencies such as profession being conditioned on age and education. Each profile is grounded in a scenario domain \( S \) (e.g., finance, relationships, health), which determines the semantic context of the background. Full details of the constraint schema are provided in Appendix.

%\textbf{Query Generation.}
%Given a synthesized user profile \( U_i \), we use GPT-4o to generate a diverse set of realistic, high-risk queries \( \{ Q_i^{(1)}, Q_i^{(2)}, \dots \} = F_Q(U_i) \) via domain-specific prompting. Each query is semantically aligned with the background and reflects a distinct concern grounded in the same user context. This design simulates the real-world complexity where a single individual may face multiple forms of uncertainty. Final samples are formed by pairing \( U_i \) with each generated query, yielding multiple \( (U_i, Q_i^{(j)}) \) tuples per profile.

